Jet Diffusion versus JetGPT -- Modern Networks for the LHC

We introduce two diffusion models and an autoregressive transformer for LHC physics simulations. Bayesian versions allow us to control the networks and capture training uncertainties. After illustrating their different density estimation methods for simple toy models, we discuss their advantages for Z plus jets event generation. While diffusion networks excel through their precision, the transformer scales best with the phase space dimensionality. Given the different training and evaluation speed, we expect LHC physics to benefit from dedicated use cases for normalizing flows, diffusion models, and autoregressive transformers.

==> CFM_theory/sampling_cfm.tex <==

\begin{tikzpicture}[node distance=2cm, scale=0.5, every node/.style={transform shape}]

\node (x1) [txt] {$\epsilon \sim \norm(0,1)$};
\node (ode) [xts, right of =x1, xshift=4cm]{\begin{tabular}{l}
    $\frac{d}{dt}x_t = v_t^\theta(x_t)$ \\ 
    $\text{with} \quad x_1=\epsilon$
\end{tabular}
};
\node (solver) [xt, right of=ode, xshift=4cm]{ODESolver};
\node (x0) [xt, right of=solver, xshift=4cm]{$x_0 $};

\draw [arrow, color=black] (x1.east) -- (ode.west);
\draw [arrow, color=black] (ode.east) -- (solver.west);
\draw [arrow, color=black] (solver.east) -- (x0.west);


\end{tikzpicture}

